Online Resynthesis of High-Level Collaborative Tasks for Robots with Changing Capabilities

Given a collaborative high-level task and a team of heterogeneous robots and behaviors to satisfy it, this work focuses on the challenge of automatically, at runtime, adjusting the individual robot behaviors such that the task is still satisfied, when robots encounter changes to their abilities--either failures or additional actions they can perform. We consider tasks encoded in LTL^\psi and minimize global teaming reassignments (and as a result, local resynthesis) when robots' capabilities change. We also increase the expressivity of LTL^\psi by including additional types of constraints on the overall teaming assignment that the user can specify, such as the minimum number of robots required for each assignment. We demonstrate the framework in a simulated warehouse scenario.

==> algorithms/update_prod_aug.tex <==
\begin{algorithm}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \SetKwProg{Initialization}{Initialization}{}{}
    \Input{$A_j$, $\mathcal{G}_j, \BuchiBeta, \Delta^{aug}_{j}$} 
    \Output{$\mathcal{G}^{upd}_j$}
    % $\gamma^{aug} = \{(s, s^*) \in S^{aug}\ | \ \exists x \in s \} \cup \{(s^*, s') \in S^{aug}\ | \ \exists x' \in s' \} $ \\
    % \For{$(x, x') \in \DeltaAug$}{
        $\{(s, s^*) \in S^{aug}\ | \ \exists x \in s, s^* = \textsc{get\_new\_state}(s, x')\}$ \\

        $\{(s^*, s) \in S^{aug}\ | \ \exists x' \in s, s^* = \textsc{get\_new\_state}(s, x)\}$
    
    % }
    
    % % $s^* = \textsc{get_new_state(s, x)}$
    % $A_j' = \textsc{get\_neighbor\_edges}(A_j, \Delta^{aug}_{j})$ \\
    % $\mathcal{G}_j' = A_j' \times \BuchiBeta$ \\
    % \tcp{join two product automata} 
    % $\mathcal{G}^{upd}_j = \mathcal{G}_j \cup \mathcal{G}_j'$ \\
    \Return $\mathcal{G}^{upd}_j$      
\caption{Update Product Automaton: augmented transitions}
\label{algo:update_prod_aug}
\end{algorithm}

==> algorithms/update_prod_fail.tex <==
\begin{algorithm}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \SetKwProg{Initialization}{Initialization}{}{}
    \Input{$\mathcal{G}_j, \BuchiBeta, \Delta^{fail}_{j}, q^t_j$} 
    \Output{$\mathcal{G}^{upd}_j$}

    $\mathcal{G}^{upd}_j = \mathcal{G}_j$ \\
    $\delta^{fail}_\mathcal{G} = \{((s,z), (s',z')) \in \delta_{\mathcal{G}, j} \ | \  (s,s') \in \Delta^{fail}_{j},$ $(z,z') \in \BuchiBeta \}$ \\
    $\delta^{upd}_{\mathcal{G}, j} = \delta_{\mathcal{G}, j} \setminus \delta^{fail}_\mathcal{G} $ \\
    \Return $\mathcal{G}^{upd}_j$
       
\caption{Update Product Automaton: Failed transitions}
\label{algo:update_prod_fail}
\end{algorithm}

==> figures/performance.tex <==
\renewcommand{\arraystretch}{1.8}   %Presets from my institute
\newcolumntype{M}{X<{\vspace{4pt}}} %Presets from my institute


\begin{table}
% \centering 
\begin{tabularx}{\columnwidth}{|p{\dimexpr.10\linewidth-2\tabcolsep-1.3333\arrayrulewidth}% column 1
  |p{\dimexpr.45\linewidth-2\tabcolsep-1.3333\arrayrulewidth}% column 2
  |p{\dimexpr.45\linewidth-2\tabcolsep-1.3333\arrayrulewidth}|% column 3} 
  }
    % \begin{tabular}{ |c|c|c| } 
     \hline
     $m$ & our allocation & optimal allocation  \\
     \hline
    4 &    6.19E-5 / (5.894E-5, 7.30E-5)	&     1.24E-5 / (1.10E-5, 1.72E-5)      \\
    5 &    6.39E-5 / (6.08E-5, 6.91E-5)      &     1.30E-5 / (1.17E-5, 1.60E-5)      \\
    6 &    6.51E-5 / (6.20E-5, 7.30E-5)      &     1.32E-5 / (1.19E-5, 1.60E-5)      \\
    7 &    7.17E-5 / (6.51E-5, 8.393E-5)     &     0.018 / (1.29E-5, 0.72)         \\
    8 &    7.68E-5 / (6.82E-5, 9.80E-5)      &     0.045 / (1.38E-5, 0.86)         \\
    9 &    7.43E-5 / (6.87E-5, 9.11E-5)      &     0.076 / (1.26E-5, 3.21)         \\
    10 &    8.10E-5 / (7.20E-5, 9.58E-5)     & 	  0.144 / (1.38E-5, 3.21) \\        
    % 4 &  0 / (0, 0) & 0 / (0, 0)\\
    % 5 & 0.01 / (0, 1) & 0 / (0, 0)\\
    % 6 & 0.006666667 / (0, 1) & 0 / (0, 0)\\
    % 7 & 0.035 / (0, 2) & 0 / (0, 0)\\
    % 8 & 0.044 / (0, 2) & 0 / (0, 0)\\
    % 9 & 0.046666667 / (0, 2) & 0 / (0, 0)\\
    % 10 & 0.57142857 / (0, 2) & 0 / (0, 0)\\
     \hline
    \end{tabularx}
    \caption{Average / (min, max) of the number of robots that are reassigned when finding a new team while varying the number of total bindings $m$.}
    \label{table:sim_performance}
\end{table}



